Nonreciprocal electromagnetic wave manipulation via a single reflection

Electric field manipulation plays a key role in applications such as electron acceleration, nonlinear light-matter interaction, and radiation engineering. Nonreciprocal materials, such as Weyl semimetals, enable the manipulation of the electric field in a full photonic manner, owing to their intrinsic time-reversal symmetry breaking, leading to asymmetric material response for photons with +k and -k momenta. Here, the results suggest that a simple planar interface between semi-infinite air and a nonreciprocal material can achieve spatio-temporal manipulation of the electric field. In particular, this work presents three compelling scenarios for electromagnetic wave manipulation: radiation pattern redistribution (with closed-form expressions provided), carrier-envelope phase control, and spatial profile control. The presented results pave the way for electric field manipulation using pattern-free nonreciprocal materials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
